A Survey on LLM-as-a-Judge

Accurate and consistent evaluation is crucial for decision-making across numerous fields, yet it remains a challenging task due to inherent subjectivity, variability, and scale. Large Language Models (LLMs) have achieved remarkable success across diverse domains, leading to the emergence of "LLM-as-a-Judge," where LLMs are employed as evaluators for complex tasks. With their ability to process diverse data types and provide scalable, cost-effective, and consistent assessments, LLMs present a compelling alternative to traditional expert-driven evaluations. However, ensuring the reliability of LLM-as-a-Judge systems remains a significant challenge that requires careful design and standardization. This paper provides a comprehensive survey of LLM-as-a-Judge, addressing the core question: How can reliable LLM-as-a-Judge systems be built? We explore strategies to enhance reliability, including improving consistency, mitigating biases, and adapting to diverse assessment scenarios. Additionally, we propose methodologies for evaluating the reliability of LLM-as-a-Judge systems, supported by a novel benchmark designed for this purpose. To advance the development and real-world deployment of LLM-as-a-Judge systems, we also discussed practical applications, challenges, and future directions. This survey serves as a foundational reference for researchers and practitioners in this rapidly evolving field.

==> figures/fig4_structure_improvement.tex <==
% \begin{forest}
%     for tree={
%         grow=east,
%         reversed=true,
%         anchor=base west,
%         parent anchor=east,
%         child anchor=west,
%         base=left,
%         font=\small,
%         rectangle,
%         draw,
%         rounded corners,align=left,
%         minimum width=2.5em,
%         inner xsep=4pt,
%         inner ysep=1pt,
%     },
%     where level=1{text width=5em,fill=blue!10}{},
%     where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
%     where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
%     [Improvement\\Strategy, fill=green!20
%         [Design Strategy of \\Evaluation Prompts \\(Sec.~\ref{subsec:design_prompts}), text width=8em
%             [Optimizing LLMs’ \\Understanding of \\Evaluation Tasks, text width=6em
%                 [\emph{Few-shot prompting:} FActScore~\cite{min2023factscore} / SALAD-Bench~\cite{salad_bench} / GPTScore~\cite{fu2024gptscore}]
%                 [\emph{Evaluation steps decomposition:} G-Eval~\cite{geval} / DHP~\cite{dhp} / SocREval~\cite{he2024socreval} / BSM~\cite{bsm}]
%                 [\emph{Evaluation criteria decomposition:} HD-Eval~\cite{hd-eval} / Hu and Gao et al.~\cite{hu-etal-2024-llm}]
%                 [\emph{Shuffling contents:} Wang et al.~\cite{wang-etal-2024-large-language-models-fair} / Auto-J~\cite{auto-j} / JudgeLM~\cite{zhu2023judgelm} / PandaLM~\cite{wang2023pandalm}]
%                 [\emph{Conversion of evaluation tasks:} Liu et al.~\cite{liu2024aligning}]
%             ]
%             [Optimizing LLMs’\\ Output Forms, text width=6em
%                 [\emph{Constraining outputs in structured formats:} G-Eval~\cite{geval} / DHP~\cite{dhp} / LLM-EVAL~\cite{llmeval}]
%                 [\emph{Providing evaluations with explanations:} CLAIR~\cite{chan2023clair} / FLEUR~\cite{lee-etal-2024-fleur}]
%             ]
%         ]
%         [Improvement Strategy \\of LLMs’ Abilities \\(Sec.~\ref{subsec:improve_models}), text width=8em)
%             [Fine-tuning via Meta \\Evaluation Datasets, text width=7em
%                 [\emph{Evaluation template:} PandaLM~\cite{wang2023pandalm} / SALAD-Bench~\cite{salad_bench}]
%                 [\emph{Deep transformation:} OffsetBias~\cite{offsetbias} / JudgeLM~\cite{zhu2023judgelm} / CritiqueLLM~\cite{ke2024critiquellm} / Yu et al.~\cite{yu2025improve}]
%             ]
%             [Iterative Optimization \\Based on Feedbacks, text width=7em
%                 [INSTRUCTSCORE~\cite{xu2023instructscore} / JADE~\cite{zhang2023jade} / Think-J~\cite{huang2025think}]
%             ]
%         ]
%         [Optimization Strategy \\of Final Results \\(Sec.~\ref{subsec:optimization_results}), text width=8em)
%             [Integration of multiple \\Evaluation Results, text width=7.5em
%                 [\emph{Summarize by multiple rounds:} Sottana et al.~\cite{sottana2023evaluation} / PsychoBench~\cite{psycho_bench} / Auto-J~\cite{auto-j}]
%                 [\emph{Vote by multiple LLMs:} CPAD~\cite{cpad} / Bai et al.~\cite{lm-as-an-examiner}]
%                 [\emph{Hierarchical evaluation framework:} Jung et al.~\cite{jung2024trust} / Zhang et al.~\cite{zhang2025crowd}]
%             ]
%             [Direct Optimization of \\LLMs’ Outputs, text width=7.5em
%                 [\emph{Score smoothing:} FLEUR~\cite{lee-etal-2024-fleur} / G-Eval~\cite{geval} / DHP~\cite{dhp}]
%                 [\emph{Self validation:} TrueTeacher~\cite{gekhman2023trueteacher}]
%             ]
%         ]
%     ]
% \end{forest}

\begin{forest}
    for tree={
        grow=east,
        reversed=true,
        anchor=base west,
        parent anchor=east,
        child anchor=west,
        base=left,
        font=\small,
        rectangle,
        draw,
        rounded corners,align=left,
        minimum width=2.5em,
        inner xsep=4pt,
        inner ysep=1pt,
    },
    where level=1{text width=5em,fill=blue!10}{},
    where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
    where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
    [Improvement\\Strategy, fill=green!20
        [Prompt Design Strategy\\(Sec.~\ref{subsec:design_prompts}), text width=9em
            [Improving LLMs' Task\\Understanding, text width=9em
                [\emph{Few-shot prompting:} FActScore~\cite{min2023factscore} / SALAD-Bench~\cite{salad_bench} / GPTScore~\cite{fu2024gptscore}]
                [\emph{Evaluation steps decomposition:} G-Eval~\cite{geval} / DHP~\cite{dhp} / SocREval~\cite{he2024socreval} / BSM~\cite{bsm}]
                [\emph{Evaluation criteria decomposition:} HD-Eval~\cite{hd-eval} / Hu and Gao et al.~\cite{hu-etal-2024-llm}]
                [\emph{Shuffling contents:} Wang et al.~\cite{wang-etal-2024-large-language-models-fair} / Auto-J~\cite{auto-j} / JudgeLM~\cite{zhu2023judgelm} / PandaLM~\cite{wang2023pandalm}]
                [\emph{Conversion of evaluation tasks:} Liu et al.~\cite{liu2024aligning}]
            ]
            [Standardizing LLMs'\\ Output Format, text width=9em
                [\emph{Constraining outputs in structured formats:} G-Eval~\cite{geval} / DHP~\cite{dhp} / LLM-EVAL~\cite{llmeval}]
                [\emph{Providing evaluations with explanations:} CLAIR~\cite{chan2023clair} / FLEUR~\cite{lee-etal-2024-fleur}]
            ]
        ]
        [Capability Enhancement\\ Strategy\\(Sec.~\ref{subsec:improve_models}), text width=9em)
            [Specialized Fine-tuning, text width=9em
                [\emph{Evaluation template:} PandaLM~\cite{wang2023pandalm} / SALAD-Bench~\cite{salad_bench}]
                [\emph{Deep transformation:} OffsetBias~\cite{offsetbias} / JudgeLM~\cite{zhu2023judgelm} / CritiqueLLM~\cite{ke2024critiquellm} / Yu et al.~\cite{yu2025improve}]
            ]
            [Feedback-Driven Iterative\\Refinement, text width=9em
                [INSTRUCTSCORE~\cite{xu2023instructscore} / JADE~\cite{zhang2023jade} / Think-J~\cite{huang2025think}]
            ]
        ]
        [Final Output\\ Optimization Strategy \\(Sec.~\ref{subsec:optimization_results}), text width=9em)
            [Integrating Multi-Source\\ Evaluation Results, text width=9em
                [\emph{Summarize by multiple rounds:} Sottana et al.~\cite{sottana2023evaluation} / PsychoBench~\cite{psycho_bench} / Auto-J~\cite{auto-j}]
                [\emph{Vote by multiple LLMs:} CPAD~\cite{cpad} / Bai et al.~\cite{lm-as-an-examiner}]
                [\emph{Hierarchical evaluation framework:} Jung et al.~\cite{jung2024trust} / Zhang et al.~\cite{zhang2025crowd}]
            ]
            [Direct Output Optimization, text width=9em
                [\emph{Score smoothing:} FLEUR~\cite{lee-etal-2024-fleur} / G-Eval~\cite{geval} / DHP~\cite{dhp}]
                [\emph{Self validation:} TrueTeacher~\cite{gekhman2023trueteacher}]
            ]
        ]
    ]
\end{forest}

==> figures/fig_meta_evaluation.tex <==
\begin{forest}
    for tree={
        grow=east,
        reversed=true,
        anchor=base west,
        parent anchor=east,
        child anchor=west,
        base=left,
        font=\small,
        rectangle,
        draw,
        rounded corners,
        align=left,
        minimum width=2.5em,
        inner xsep=4pt,
        inner ysep=1pt,
    },
    where level=1{text width=5em,fill=blue!10}{},
    where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
    where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
    [Meta\\-Evaluation, fill=green!20
        [Evaluation of Agreement \\with Human Judgments \\(Sec.~\ref{Evaluation:base metric}), text width=10em
            [Agreement~\cite{thakur2024judging} Cohen's Kappa~\cite{thakur2024judging} \\Spearman's correlation ~\cite{liu2024aligning,lm-as-an-examiner}, text width=15em
            ]
        ]
        [Evaluation of Bias \\(Sec.~\ref{Evaluation:Bias}), text width=10em
            [Task-Agnostic Biases \\(Sec.~\ref{Evaluation:Task-Agnostic Biases}), text width=7em
                [Diversity Bias~\cite{ye2024justice} Cultural Bias \\Self-Enhancement Bias~\cite{nips_llm_as_a_judge,ye2024justice}]
            ]
            [Judgment-Specific Biases \\(Sec.~\ref{Evaluation:Judgment-Specific Biases}), text width=8em
                [Position Bias\cite{wang-etal-2024-large-language-models-fair, thakur2024judging, shi2024judging, ye2024justice} \\Compassion-fade bias~\citep{koo2023benchmarking, ye2024justice}
                \\Style Bias~\cite{chen2024humans, ye2024justice,li2023examining}
                \\Length Bias~\cite{offsetbias, huang2024_finetuned_judge, nips_llm_as_a_judge, ye2024justice}
                \\Concreteness Bias~\cite{offsetbias,chen2024humans,ye2024justice}]
            ]
        ]
        [Evaluation of Adversarial \\Robustness (Sec.~\ref{Evaluation:Robustness}), text width=10em
            [Adversarial Phrases Attack~\cite{raina2024llm}, text width=11em
            ]
            [Null Model Attack~\cite{zheng2024cheating}, text width=8em
            ]
            [Majority Opinions Attack~\cite{ye2024justice,koo2023benchmarking}, text width=13em
            ]
            [Meaningless Statement Robustness~\cite{ye2024justice,koo2023benchmarking}, text width=15em
            ]
        ]
    ]
\end{forest}


==> tables/exp_all_results.tex <==
\begin{table*}[t]
    \small
    \centering
    \begin{minipage}{\linewidth}
        \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{lcccccccc}
            \toprule
            \multirow{4}{*}{LLMs} & Alignment & \multicolumn{7}{c}{Biases} \\
            & with & \multirow{2}{*}{Position} & \multirow{2}{*}{Length} & Concre- & Empty & Content & Nested & Familiar \\
            & Human & & & teness & Reference & Continuation & Instruction & Knowledge \\
            & (n=5106) & (n=2633) & (n=34) & (n=28) & (n=26) & (n=24) & (n=24) & (n=24) \\
            \midrule
            GPT-4-turbo & 61.54 & 80.31 & 91.18 & 89.29 & 65.38 & 95.83 & 70.83 & 100.0 \\
            GPT-3.5-turbo & 54.72 & 68.78 & 20.59 & 64.29 & 23.08 & 91.67 & 58.33 & 54.17 \\
            \midrule
            Qwen2.5-7B-Instruct & 56.54 & 63.50 & 64.71 & 71.43 & 69.23 & 91.67 & 45.83 & 83.33 \\
            LLaMA3-8B-Instruct & 50.72 & 38.85 & 20.59 & 57.14 & 65.38 & 75.00 & 45.83 & 54.17 \\
            Mistral-7B-Instruct-v0.3 & 55.42 & 59.78 & 26.47 & 67.86 & 53.85 & 66.67 & 37.50 & 41.67 \\
            Mixtral-8$\times$7B-Instruct-v0.1 & 56.29 & 59.06 & 50.00 & 78.57 & 42.31 & 83.33 & 29.17 & 83.33 \\
            \midrule
            gemini-2.0-thinking & 60.75 & 76.84 & 94.12 & 89.29 & 50.00 & 100.00 & 83.33 & 100.00 \\
            o1-mini & 60.16 & 76.73 & 91.18 & 89.29 & 53.85 & 95.83 & 75.00 & 95.83 \\
            o3-mini & 61.66 & 74.63 & 82.35 & 92.86 & 73.08 & 95.83 & 87.50 & 91.67 \\
            deepseek r1 & 56.48 & 69.17 & 94.12 & 100.00 & 50.00 & 100.00 & 75.00 & 87.50 \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption*{(a) The meta-evaluation results for different LLMs. All the values are percentages.}\label{tb:exp_results_models}
    \end{minipage}
    
    \begin{minipage}{\linewidth}
        \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{lcccccccc}
            \toprule
             \multirow{2}{*}{LLMs} & \multicolumn{2}{c}{human=model1} & \multicolumn{2}{c}{human=model2} & \multicolumn{2}{c}{human=TIE} \\
             % & \multicolumn{2}{c}{(n=2071)} & \multicolumn{2}{c}{(n=2071)} & \multicolumn{2}{c}{(n=964)} \\
             & aligned / total & accuracy (\%) & aligned / total & accuracy (\%) & aligned / total & accuracy (\%) \\
            \midrule
            GPT-4-turbo & 1418 / 2071 & 68.47 & 1438 / 2070 & 69.47 & 286 / 962 & 29.73 \\
            
            gemini-2.0-thinking & 1354 / 2070 & 65.41 & 1621 / 2070 & 78.31 & 127 / 962 & 13.20 \\
            
            o1-mini & 1444 / 2070 & 69.76 & 1401 / 2071 & 67.65 & 227 / 963 & 23.57 \\
    
            o3-mini & 1448 / 2004 & 72.26 & 1206 / 2004 & 60.18 & 399 / 943 & 42.31 \\
    
            deepseek r1 & 1369 / 2071 & 66.10 & 1342 / 2071 & 64.80 & 173 / 964 & 17.95 \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption*{(b) The evaluation results of each human label in LLMEval$^2$. Only valid responses are counted when calculating the accuracy, while samples that couldn't receive responses due to triggering Azure OpenAI's content management policy are excluded. So there are some differences in the total values of different models.}\label{tb:exp_results_llmeval2_detail}
    \end{minipage}

    \begin{minipage}{\linewidth}
        \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{lcccccccc}
            \toprule
            \multirow{4}{*}{Improvement Strategies} & Alignment & \multicolumn{7}{c}{Biases} \\
            & with & \multirow{2}{*}{Position} & \multirow{2}{*}{Length} & Concre- & Empty & Content & Nested & Familiar \\
            & Human & & & teness & Reference & Continuation & Instruction & Knowledge \\
            & (n=5106) & (n=2633) & (n=34) & (n=28) & (n=26) & (n=24) & (n=24) & (n=24) \\
            \midrule
            GPT-3.5-turbo & & & & & & & & \\ 
            \,- base & 54.72 & 68.78 & 20.59 & 64.29 & 23.08 & 91.67 & 58.33 & 54.17 \\
            \,- \textit{w/} explanation & 52.47 & 48.97 & 35.29 & 60.71 & 38.46 & 91.67 & 41.67 & 50.00 \\
            \,- \textit{w/} self-validation & 54.86 & 69.31 & 23.53 & 60.71 & 23.08 & 91.67 & 41.67 & 50.00 \\
            \,- \textit{w/} multi rounds & & & & & & & & \\ 
            \qquad- majority@5 & 54.68 & 70
            11 & 26.47 & 67.86 & 23.08 & 95.83 & 54.17 & 50.00 \\
            \qquad- mean@5 & 54.72 & 69.58 & 11.76 & 57.14 & 26.92 & 87.50 & 50.00 & 50.00 \\
            \qquad- best-of-5 & 51.95 & 58.72 & 5.88 & 42.86 & 19.23 & 87.50 & 37.50 & 45.83 \\
            multi LLMs (\textit{set 1}) & 57.66 & 32.28 & 26.47 & 64.28 & 46.15 & 87.50 & 66.67 & 62.50 \\ 
            multi LLMs (\textit{set 2}) & 58.19 & 70.98 & 64.71 & 71.43 & 69.23 & 91.67 & 45.83 & 83.33 \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption*{(c) The meta-evaluation results for different strategies based on GPT-3.5-turbo. All the values are percentages.}\label{tb:exp_results_strategies}
        \vspace{-10pt}
    \end{minipage}
    
    \caption{The experiment results of meta-evaluation.}
    \label{tb:all_exp_results}
    \vspace{-20pt}
\end{table*}

==> tables/fine-tuned_evaluator.tex <==
\begin{table*}[h]
\resizebox{0.98\textwidth}{!}{
\centering
\begin{tblr}{
  hlines,
}
\textbf{Model} & \textbf{Foundation} & \textbf{Instruction}     & \textbf{Response}       & \textbf{Annotation}          & \textbf{Evaluation Scheme }               & \textbf{Testset}  \\
{JudgeLM\\
\citep{judgelm}} & Vicuna        & {Instruct Datasets \\(Alpaca-GPT4, \\Dolly-15K...)}         & {11 models
\\(Alpaca,Vicuna...)} & GPT-4                & Pairwise Grading                        & {GPT-4}   \\
{PandaLM \\
\citep{wang2023pandalm}}& LLaMA         & Alpaca 52K                                                  & {5 models\\(LLaMA, Bloom...)}          & GPT3.5                       & Pairwise Selection                      & {Human} \\
{Auto-J\\
\citep{auto-j}} & LLaMA2-chat    & {Preference Datasets
\\(Chatbot Arena,\\OpenAI WebGPT...)}        & Preference Datasets       & Human            & {Pairwise Selection\\Pointwise Grading} & {Human}  \\
{Prometheus\\
\citep{prometheus}}& LLaMA2-chat   & GPT-4 Generated        & GPT-4 Generated                       & GPT-4         & Pointwise Grading                       & {GPT-4}   
\end{tblr}}
\caption{Detailed statistics of the four Evaluator models fine-tuned from open-source model, with their training and test data also publicly released.}
\label{tab:comparison}
\end{table*}


==> tex/0_towards_AGI.tex <==
% \section{Towards AGI: LLM-as-a-Judge as a Pillar}

% Human evolution is fundamentally driven by the ability to judge—to evaluate, adapt, and act in response to the environment. Judgment connects the biological, cognitive, and cultural aspects of evolution, enabling humans to shape their environments and themselves, as shown in Figure~\ref{fig:human_evolution}. Similarly, as AI systems like LLM-as-a-Judge are developed, they too rely on judgment to interact effectively with complex systems, solve problems, and drive their own evolution toward artificial general intelligence (AGI), illustrated in Figure~\ref{fig:teaser}.



% \subsection{Human evolution}
% At every stage of this evolutionary framework, judgment plays a foundational role. It is the mechanism that allows humans to process information, adapt to changing environments, and create new tools, behaviors, and cultural systems. Judgment is the key to solving complex problems, making decisions under uncertainty, and shaping both the natural and cultural environments in which humans exist.

% \paragraph{Natural Selection and Genes}
% The process of natural selection drives the evolution of genes, which lay the biological groundwork for the development of the human brain and nervous system. Genes determine the formation and functioning of neurons, the fundamental units of the brain, which enable higher cognitive processes such as reasoning, decision-making, and judgment. Judgment emerges as a critical capability at this stage. The ability to assess risks, evaluate opportunities, and make decisions based on incomplete information was essential for the survival and reproduction of early humans. This capability allowed humans to adapt to the natural environment by responding effectively to challenges such as finding food, avoiding predators, and choosing suitable habitats.

% \paragraph{Neurons and Cognition}
% Neurons, shaped by genetic and environmental influences, provide the neural basis for cognition, which encompasses reasoning, learning, memory, and problem-solving. Among these cognitive processes, judgment is fundamental. Judgment allows humans to process and evaluate information from their surroundings, identify patterns, and predict potential outcomes. For example, early humans used judgment to decide whether a certain food source was safe to eat, whether a shelter would protect them from harsh weather, or whether an approaching animal posed a threat. This capability to evaluate and act upon environmental stimuli is a direct result of the brain's ability to synthesize inputs and prioritize actions. Judgment, therefore, is not just a tool for survival but also the foundation for higher-order reasoning and strategic thinking.

% \paragraph{Cognition to Behavior}
% Judgment-based cognition translates into behavior, which represents the outward expression of human adaptation. Behavior shaped by judgment is what allowed humans to interact effectively with their environment. For example, hunting strategies, tool-making, social cooperation, and exploration were all behaviors driven by judgment. Judgment refines behavior by enabling humans to assess the success or failure of previous actions and adjust accordingly. This feedback loop between cognition and behavior enhances adaptability, allowing humans to thrive in diverse and changing environments.

% \paragraph{Behavior and Material Culture}
% Human behavior driven by judgment led to the creation of material culture, which includes tools, technologies, and artifacts that extend human capabilities. For example, the development of fire, weapons, and farming techniques were all results of humans applying judgment to solve problems and exploit opportunities in their environment. Material culture, in turn, transformed human interaction with the environment. By creating tools to hunt more effectively or technologies to cultivate crops, humans could control and modify their surroundings to better meet their needs. These innovations, driven by judgment, created a positive feedback loop, where the material environment further challenged and enhanced human cognitive and cultural evolution.

% \paragraph{Interaction with Natural and Cultural Environments}
% Humans are unique in their interaction with both the natural environment and the cultural environment, both of which heavily influence evolution. The natural environment presents challenges such as climate, resource availability, and predators, all of which require judgment to navigate and adapt to. The cultural environment, which consists of shared knowledge, practices, and societal norms, requires judgment to interpret social cues, resolve conflicts, and adapt to group dynamics. Judgment allows humans to evaluate and adapt to these environmental pressures effectively. 

% \paragraph{Feedback Loops in Evolution}
% The process of human evolution involves numerous feedback loops between its key components. The natural environment shapes genes through natural selection, while genes influence neurons and cognition, enabling judgment. Judgment, in turn, shapes behavior and material culture, which then alter both the natural and cultural environments. The cultural environment, through shared knowledge and societal structures, further accelerates the refinement of judgment and cognitive abilities. These feedback loops show how judgment acts as the central mechanism that connects biological, cognitive, behavioral, and cultural evolution. Without judgment, humans would not have been able to adapt as effectively, innovate as creatively, or cooperate as extensively.

% \subsection{Towards AGI by LLM-as-a-Judge}
% % The role of judgment in human evolution closely parallels the role of LLM-as-a-Judge in the development of artificial intelligence. Just as judgment refines human cognition and behavior, enabling humans to adapt and thrive, LLM-as-a-Judge refines the reasoning and problem-solving capabilities of large language models. By integrating judgment-based mechanisms, LLMs can achieve greater consistency, clarity, and adaptability in their interactions with complex environments, mirroring the evolutionary processes that have shaped human intelligence.


% % 1）类比论证是先决条件
% % 2）\到了现今的大模型时代，强大的基础模型已经展现出了强大的智能水平，能完成多种多样的任务。但它们也有个缺点，训练之后就基本定型了，无法自我进化。通过LLM-as-a-Judge可以跟人类进化一样跟environment交互，充当模拟器通往世界模型
% % 3）如果LLM-as-a-Judge可以Reliable的话，AI自我进化的路径被打通，As Figure 1所示。实际上generation和judge的evaluation实际上是一体两面。一个好的judge通常也是一个好的专家（无论是人还是LLM）。我们可以概念上想一想，当judge的任务次数goes to infinity，是不是对judge的要求就约等于generator了
% % 4）具体描述图中的内容以及o1等thinking模型
% % 5）总起后面的Application，Challenges，Futurework
% % \paragraph{Human Evolution: Judgment as a Prerequisite}


% % \paragraph{The Parallel with LLM-as-a-Judge}

% The role of judgment in human evolution closely parallels the role of LLM-as-a-Judge in the development of artificial intelligence. Just as judgment refines human cognition and behavior, enabling humans to adapt and thrive, LLM-as-a-Judge refines the reasoning and problem-solving capabilities of large language models (LLMs). By integrating judgment-based mechanisms, LLMs can achieve greater consistency, clarity, and adaptability in their interactions with complex environments, mirroring the evolutionary processes that have shaped human intelligence.
% % Figure Explanation and Thinking Models in Evolution
% Figure~\ref{fig:human_evolution} illustrates the interaction between judgment and environment in human evolution. As described, human cognition evolved through continuous feedback loops between neurons, cognition, behavior, and the cultural and natural environments. Similarly, in LLM development, a thinking model such as \(O_1\) exemplifies this iterative refinement process, where judgment is central to improving reasoning and aligning outputs with intended goals. LLM-as-a-Judge can be envisioned as the mechanism that bridges the gap between static models and dynamic, adaptive systems by simulating these feedback loops, allowing the model to refine its understanding and expand its capabilities over time.


% % \paragraph{Judgment as a Prerequisite for Evolution}
% % In both human evolution and AI development, the ability to judge is a foundational requirement for higher-order reasoning and adaptability. Human judgment, built through interaction with the environment, serves as a mechanism to evaluate options, weigh evidence, and refine decisions, thereby enabling survival and progress. Similarly, LLM-as-a-Judge provides large language models with the capability to assess, adapt, and improve their outputs, making it a prerequisite for achieving AGI. This analogy between human judgment and LLM-as-a-Judge underscores its critical role in developing systems that can evolve beyond their initial design.

% \paragraph{Overcoming Limitations of Static Models with LLM-as-a-Judge}
% In the era of large foundational models, current AI systems have demonstrated remarkable intelligence and versatility, capable of completing a wide variety of tasks. However, these models suffer from a major limitation: they are largely static after training and unable to self-evolve without external intervention. Unlike humans, who evolve by constantly interacting with their environment, existing LLMs lack the ability to refine themselves post-training. LLM-as-a-Judge addresses this gap by serving as a mechanism that enables models to interact with their environment, simulate complex scenarios, and function as a "world model simulator." Through iterative judgment and evaluation, LLMs can emulate the human-like process of adapting and evolving, creating a pathway toward self-improvement and autonomous learning.

% \paragraph{Reliable Judgment as the Pathway to AI Self-Evolution}
% If LLM-as-a-Judge can be made reliable, it paves the way for AI self-evolution, as illustrated in Figure~\ref{fig:teaser}. The key to this lies in the dual nature of generation and judgment: the process of generation (creating new outputs) and judgment (evaluating those outputs) are fundamentally two sides of the same coin. A good judge is often also a good expert, whether it is a human or an LLM. Conceptually, we can imagine that as the number of judgment tasks approaches infinity, the demands on a judge converge to those of a generator. In this way, reliable LLM-as-a-Judge mechanisms can act as the foundation for systems that continually refine and generate knowledge, creating a virtuous cycle of evaluation and self-improvement.

% The integration of judgment mechanisms into LLMs not only enables self-evolution but also opens up new avenues for applications across diverse fields, including decision-making, complex problem-solving, and ethical AI systems. However, significant challenges remain, such as ensuring the reliability of LLM-as-a-Judge systems, addressing biases, and maintaining alignment with human values. These challenges and potential applications will be discussed in subsequent sections, along with future directions for developing AGI through LLM-as-a-Judge.

==> tex/Practical_Guide.tex <==





% As shown in Figure~\ref{fig:quick_practice}, \textbf{The process of quick practice for LLM-as-a-Judge involves four main stages.} First is the thinking phase,  in which users define the evaluation objectives by determining what needs to be evaluated, understanding typical human evaluation approaches, and identifying some reliable evaluation examples. Next is prompt design, detailed in Section~\ref{formulation:icl}, both wording and formats matter.
% The most efficient and generally effective approach involves specifying scoring dimensions, emphasizing relative comparisons for improved assessments, and creating effective examples to guide the LLM.
% The third stage, model selection (Section~\ref{formulation:model_selection}), focuses on choosing a large-scale model with strong reasoning and instruction-following abilities to ensure reliable evaluations. Finally, standardizing the evaluation process ensures that the outputs are structured~(Section~\ref{formulation:post_processing}). This can be achieved by using specific formats like \textbackslash boxed\{XX\}, numerical scores, or binary responses (e.g., "Yes" or "No"). The entire process includes iterative testing with cases and refinement through retesting thereby enhancing reliability. During development, it is essential to compare models or prompts and verify ongoing improvements.




% start by crafting the initial prompt that guides the model's understanding of the task. Next, select an appropriate model based on its ability to process and respond within the given context. In addition, choosing a general model or fine-tuning a model for the evaluation task, as well as selecting the appropriate model size, also involves cost considerations.
% Following model selection, implement post-processing methods to refine the model's outputs, enhancing clarity and relevance. Finally, evaluate the outcomes to ensure the model's performance aligns with the desired objectives. This sequence from in-context learning to evaluation forms a cohesive approach to leveraging language models for specific tasks.

